RIS-Enabled NLoS Near-Field Joint Position and Velocity Estimation under User Mobility

In the context of single-base station (BS) non-line-of-sight (NLoS) single-epoch localization with the aid of a reflective reconfigurable intelligent surface (RIS), this paper introduces a novel three-step algorithm that jointly estimates the position and velocity of a mobile user equipment (UE), while compensating for the Doppler effects observed in near-field (NF) at the RIS elements over the short transmission duration of a sequence of downlink (DL) pilot symbols. First, a low-complexity initialization procedure is proposed, relying in part on far-field (FF) approximation and a static user assumption. Then, an alternating optimization procedure is designed to iteratively refine the velocity and position estimates, as well as the channel gain. The refinement routines leverage small angle approximations and the linearization of the RIS response, accounting for both NF and mobility effects. We evaluate the performance of the proposed algorithm through extensive simulations under diverse operating conditions with regard to signal-to-noise ratio (SNR), UE mobility, uncontrolled multipath and RIS-UE distance. Our results reveal remarkable performance improvements over the state-of-the-art (SoTA) mobility-agnostic benchmark algorithm, while indicating convergence of the proposed algorithm to respective theoretical bounds on position and velocity estimation.

==> Notes.tex <==
\begin{comment}
    in this file, I will state some of the points to look for and fix by the end of writing the paper. Make sure:
    1. all the acronyms are well defined
    2. to use \ac command/s
    3. all the reference are homogeneous
    4. to well define what is algorithm 1,2,3 and how to use them
    5. Figures or Figs?
    by Moustafa Rahal
\end{comment}

==> Sections/6D_est.tex <==
\section{Position and Velocity Estimates with Zero Prior Knowledge}
\label{sec:6DEstimate}

Finally, in this section, we propose algorithm~\ref{alg4:overall} which elaborates the overall procedure of estimating the 6D position and velocity parameters of the mobile \ac{UE} with zero prior knowledge.

It commences by assuming a static \ac{UE} with unknown position and implementing algorithm~\ref{alg1:init_pos} to run a 2D and then 1D grid searches. The output of algorithm~\ref{alg1:init_pos}, i.e., faulty initial position and channel gain estimates, is then passed directly to algorithm~\ref{alg3:ref_vel} to correct the velocity (and channel gain) estimate. After that, we iteratively refine both position and velocity estimates by means of algorithms~\ref{alg2:ref_pos} $\&$ \ref{alg3:ref_vel} respectively until the objective function~\ref{eq:ml_pos_vel_gain} converges. A final, Quasi-Newton, refinement routine is performed to better estimate the positional, velocity, and gains parameters.
\begin{algorithm}
	\caption{6D Estimation in RIS-Aided Near-Field Localization: $(\alphahat, \pphat, \vvhat) = \findposvel(\yy)$}
% 	\footnotesize
	\begin{algorithmic}[1]
	    \State \textbf{Input:} Observation $\yy$ in \eqref{eq:yy}.
	    \State \textbf{Output:} Position, velocity and gain estimates $\alphahat, \pphat, \vvhat$.
	    \State Initialize the velocity estimate as $\vvhat = \boldzero \unit{m/s}$.
	    \State Initialize the position and gain estimates via algorithm~\ref{alg1:init_pos}:
	    \begin{align}
	        (\pphat, \alphahat) = \initposgain(\yy) ~. \nonumber
	    \end{align}
	    \State \textbf{While} the objective in \eqref{eq:ml_pos_vel_gain} does not converge
	     \Indent
	        \State Update the velocity and gain estimates via algorithm~\ref{alg3:ref_vel}:
	        \begin{align}
	            (\vvhat,\alphahat) \leftarrow \revel(\yy, \vvhat, \pphat, \alphahat) ~. \nonumber
	        \end{align}
	        \State Update the position and gain estimates via Algorithm~\ref{alg2:ref_pos}:
	        \begin{align}
	            (\pphat, \alphahat) \leftarrow \reposgain(\yy, \vvhat, \pphat, \alphahat)~. \nonumber
	        \end{align}
	     \EndIndent
	     \State \textbf{end while} 
	     \State Perform 6D gradient descent search in \eqref{eq:ml_pos_vel} starting from $(\pphat, \vvhat)$.
	     \State Update $\alphahat$ via \eqref{eq:alphahat_update}.
	\end{algorithmic}
	\normalsize
    \label{alg4:overall}
\end{algorithm}

==> Sections/complexity_detailed.tex <==
\subsection{Algorithm~\ref{alg:init_pos}}
First we will explain the complexity of Algorithm~\ref{alg:init_pos}.
\begin{itemize}
    \item Line 1: let $K_1$, $K_2$, and $K_3$ are, resp., the search grids of $\theta$, $\phi$ and $\rho$.
    \item solving~\ref{eq:2D_ff} costs $\mathcal{O}(LM K_1 K_2)$.
    \item solving~\ref{eq:1D_distance} and~\ref{eq:2D_nf} costs $\mathcal{O}(LMK_3)$ and $\mathcal{O}(LM K_1 K_2)$, resp.
    \item given that the loop iterates $I_1$ times, then the total cost of this algorithm is $\mathcal{O}(LM I_1 \max\{K1 K_2, K_3\})$.
\end{itemize}
\subsection{Algorithm~\ref{alg:ref_pos}}
We then compute the complexity of Algorithm~\ref{alg:ref_pos}.
\begin{itemize}
    \item we first introduce $I_2$, the index of the \emph{while} loop.
    \item computing $\etab$ costs $\mathcal{O}(LM)$, so does computing $\bxib$.
    \item computing $\pdhat$ from~\ref{eq:pdhat} costs $\mathcal{O}(L)$.
    \item getting $\alphahat$ from~\ref{eq:alphahat_p} has a cost of $\mathcal{O}(L)$.
    \item the overall time complexity cost of this algorithm is $\mathcal{O}(I_2 LM)$
\end{itemize}
\subsection{Algorithm~\ref{alg:ref_vel}}
Similar to Algorithm~\ref{alg:ref_pos}, the time complexity of Algorithm~\ref{alg:ref_vel} can be computed as $\mathcal{O}(I_3 LM)$.
\subsection{Algorithm~\ref{alg:overall}}
Finally, the time complexity of Algorithm~\ref{alg:overall}.
\begin{itemize}
    \item running the algorithm in line 4 costs, as previously mentioned $\mathcal{O}(LM I_1 \max\{K_1 K_2, K_3\})$.
    \item now introducing $I_3$ as the \emph{while} index, the cost of this loop is $\mathcal{O}(I_3 LM)$.
    \item in line 9, we have a GD step which usually costs $\mathcal{O}(In^2)$ where $I$ is the number of iterations and $n$ is the number of features, which is constant in our case. So, the complexity cost of such an operation is $\mathcal{O}(I_4 ML)$, since the complexity of solving the objective function~\eqref{eq:ml_pos_vel} is $\mathcal{O}(I_4 ML)$.
    \item then the overall cost of this algorithm is$\mathcal{O}(LM (I_1 \max\{K_1 K_2, K_3\} + I_3 + I_4) )$.
\end{itemize}

==> Sections/temp.tex <==

\begin{align*}
    \widehat{\pp_\delta} &  = \frac{1}{\abs{\widehat{\alpha}}^2} \big( Re{\vect{\Xi}^\conj \vect{\Xi}^\top} \big)^{-1} Im{ \vect{\Xi}\big(    \abs{\widehat{\alpha}}^2 \vect{\eta}^\conj   -  \widehat{\alpha} \yy^\conj  \big)} ~, \\
     \widehat{\alpha}&  = \frac{ (\vect{\eta}+ j \vect{\Xi}^\top \widehat{\pp_\delta} )^\h \yy }{ \norm{\vect{\eta}+ j \vect{\Xi}^\top \widehat{\pp_\delta}}^2 }.
\end{align*}

==> figures/loc_err_vs_dist.tex <==
\begin{tikzpicture}

\begin{axis}[%
width=10cm,
height=7.4cm,
at={(0.758in,0.481in)},
scale only axis,
yminorgrids,
xmajorgrids,
xmin=1,
xmax=8,
xtick = {1, 2, 3, 4, 5, 6, 7, 8},
xlabel style={font=\color{white!15!black}},
xlabel={RIS-UE distance ($\mathrm{m}$)},
ymode=log,
ymin=0.01,
ymax=10,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={PEB ($\mathrm{m}$)},
axis background/.style={fill=white},
  legend columns=1, legend pos = north west,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color= green, line width = 1.2pt ]
  table[row sep=crcr]{
1         0.0107\\
2         0.0603\\
3         0.1661\\
4         0.3408\\
5         0.5953\\
6         0.9390\\
7         1.3804\\
8         1.9274\\
};
\addlegendentry{PEB at $v = 0~\mathrm{m/s}$}
\addplot [color=blue, line width = 1.2pt]
  table[row sep=crcr]{
1             0.0034\\
2             0.0176\\
3             0.0478\\
4             0.0973\\
5             0.1694\\
6             0.2666\\
7             0.3914\\
8             0.5459\\
};
\addlegendentry{PEB at $v = 2~\mathrm{m/s}$}
\addplot [color=red, line width = 1.2pt]
  table[row sep=crcr]{
1         0.0018\\
2         0.0073\\
3         0.0182\\
4         0.0358\\
5         0.0611\\
6         0.0952\\
7         0.1387\\
8         0.1926\\
};
\addlegendentry{PEB at $v = 6~\mathrm{m/s}$}
%\addplot [color=red, dotted, line width = 1.2pt ]
%  table[row sep=crcr]{
%1           0.302\\
%2           0.229\\
%3           0.237\\
%4           0.142\\
%5           0.191\\
%6           0.250\\
%7           4.086\\
%8           0.265\\
%};
%\addlegendentry{RMSE of alg 1 at $v = 2\mathrm{m/s}$}
%
%\addplot [color=red, dashed, line width = 1.2pt ]
%  table[row sep=crcr]{
%1           0.276\\
%2           0.185\\
%3           0.174\\
%4           0.056\\
%5           0.143\\
%6           0.201\\
%7           19.507\\
%8           0.075\\
%};
%\addlegendentry{RMSE of alg. 2 at $v = 2\mathrm{m/s}$}
%
%\addplot [color=red, line width = 1.2pt ]
%  table[row sep=crcr]{
%1           0.00006\\
%2           0.00099\\
%3           0.00830\\
%4           0.00284\\
%5           0.02697\\
%6           0.01612\\
%7           10.29064\\
%8           0.08701\\
%};
%\addlegendentry{RMSE after quasi-Newton refinement}
%
\end{axis}
\end{tikzpicture}%

%%% old curves: rmse after alg2 vs. PEB for dist = [1:4 6:2:10 15]m and v = 1 or 10 m/s
\begin{comment}
    \addplot [color=blue, line width = 1.2pt]
  table[row sep=crcr]{%
1           0.0008\\
2           0.0125\\
3           0.0668\\
4           0.2009\\
6           0.7627\\
8           1.7596\\
10          3.2948\\
15          10.2898\\
};
\addlegendentry{PEB at $v = 1\mathrm{m/s}$}

\addplot [color=blue, dashed, line width = 1.2pt]
  table[row sep=crcr]{%
1               0.0004\\
2               0.0017\\
3               0.0087\\
4               0.0405\\
6               0.8673\\
8               0.6760\\
10              0.8580\\
15              1.9791\\
};
\addlegendentry{PEB at $v = 10\mathrm{m/s}$}


\addplot [color=red , line width = 1.2pt ]
  table[row sep=crcr]{%
1               0.052\\
2               0.145\\
3               0.241\\
4               0.304\\
6               0.940\\
8               2.205\\
10              4.069\\
15              11.39\\
};

\addlegendentry{RMSE at $v = 1\mathrm{m/s}$}
%
\addplot [color=red , dashed, line width = 1.2pt ]
  table[row sep=crcr]{%
1               0.500\\
2               0.374\\
3               0.297\\
4               0.363\\
6               1.227\\
8               1.170\\
10              1.372\\
15              3.230\\
};
\addlegendentry{RMSE at $v = 10\mathrm{m/s}$}

\addplot [color= green, dashed , line width = 1.2pt ]
  table[row sep=crcr]{
1               0.671\\
2               0.553\\
3               0.497\\
4               0.541\\
6               1.084\\
8               2.371\\
10              4.590\\
15              13.333\\
};
\addlegendentry{RMSE - no velocity - $v = 10\mathrm{m/s}$}
\end{comment}

==> figures/unused/alg1_obj26_conv.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=4.521in,
height=3.566in,
at={(0.758in,0.481in)},
scale only axis,
xmin=1,
xmax=10,
xlabel style={font = \large, font=\color{white!15!black}},
xlabel={Number of Iterations},
%ymode=log,
ymin=2.54e-06,
ymax=2.61e-06,
yminorticks=true,
ylabel style={font = \large, font=\color{white!15!black}},
ylabel={Objective Function},
axis background/.style={fill=white},
% title style={font=\bfseries},
% title={Algorithm 1 - Rate of Convergence},
xmajorgrids,
ymajorgrids,
yminorgrids,
legend style={font = \large, at={(0.97,0.83)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=blue, line width=1.2pt, mark=asterisk, mark options={solid, blue}]
  table[row sep=crcr]{%
1	2.615e-06\\
2	2.549e-06\\
3	2.547e-06\\
4	2.547e-06\\
5	2.547e-06\\
6	2.547e-06\\
7	2.547e-06\\
8	2.547e-06\\
9	2.547e-06\\
10	2.547e-06\\
};
\addlegendentry{Objective Function (26)}

\end{axis}

\begin{axis}[%
width=5.833in,
height=4.375in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left
]
\end{axis}
\end{tikzpicture}%

==> figures/unused/alg4_obj13_conv.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
\definecolor{amber}{rgb}{1.00000,0.75,0.00000}%

\begin{tikzpicture}
\begin{axis}[%
width=4.521in,
height=1.566in,
at={(0.758in,2.8in)},
scale only axis,
xmin=1,
xmax=100,
xlabel style={font = \large, font=\color{white!15!black}},
xlabel={Number of Iterations},
xmode=log,
ymin=2.54e-06,
ymax=2.61e-06,
%yminorticks=true,
ylabel style={font = \large, font=\color{white!15!black}},
ylabel={Objective Function},
axis background/.style={fill=white},
title style={font=\bfseries},
title={(a) Algorithm~\ref{alg1:init_pos} Rate of Convergence},
xmajorgrids,
ymajorgrids,
yminorgrids,
xminorgrids,
legend style={font = \large, at={(0.97,0.73)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=red, line width=1.2pt]
  table[row sep=crcr]{%
1	2.615e-06\\
2	2.549e-06\\
3	2.547e-06\\
4	2.547e-06\\
5	2.547e-06\\
6	2.547e-06\\
7	2.547e-06\\
8	2.547e-06\\
9	2.547e-06\\
10	2.547e-06\\
11	2.547e-06\\
13	2.547e-06\\
14	2.547e-06\\
15	2.547e-06\\
16	2.547e-06\\
17	2.547e-06\\
18	2.547e-06\\
19	2.547e-06\\
20	2.547e-06\\
21	2.547e-06\\
22	2.547e-06\\
23	2.547e-06\\
24	2.547e-06\\
25	2.547e-06\\
26	2.547e-06\\
27	2.547e-06\\
28	2.547e-06\\
30	2.547e-06\\
32	2.547e-06\\
36	2.547e-06\\
46	2.547e-06\\
100 2.547e-06\\
};
\addlegendentry{Objective Function 26}
\end{axis}


\begin{axis}[%
width=4.521in,
height=1.566in,
at={(0.758in,0.481in)},
scale only axis,
xmin=1,
xmax=100,
xlabel style={font = \large, font=\color{white!15!black}},
xlabel={Number of Iterations},
ymode=log,
xmode=log,
ymin=1e-09,
ymax=1e-06,
yminorticks=true,
ylabel style={font = \large, font=\color{white!15!black}},
ylabel={Objective Function},
axis background/.style={fill=white},
title style={font=\bfseries},
title={(b) Algorithm~\ref{alg4:overall} Rate of Convergence},
xmajorgrids,
ymajorgrids,
yminorgrids,
xminorgrids,
legend style={font = \large, at={(0.97,0.73)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=amber, line width=1.2pt]
  table[row sep=crcr]{%
1	4.21784065056705e-07\\
2	2.54264378754792e-07\\
3	1.58855826797792e-07\\
4	1.03895808273926e-07\\
5	7.1268711115622e-08\\
6	5.08805293583305e-08\\
7	3.74108953599526e-08\\
8	2.80829153423492e-08\\
9	2.13819239870115e-08\\
10	1.6431273622503e-08\\
11	1.26970582366914e-08\\
13	7.64131822522012e-09\\
14	5.94676430181896e-09\\
15	4.64932999425744e-09\\
16	3.667390053599e-09\\
17	2.93579584028949e-09\\
18	2.40046264062052e-09\\
19	2.01587032684449e-09\\
20	1.74417722281482e-09\\
21	1.55486777213491e-09\\
22	1.42427074791603e-09\\
23	1.33474551854241e-09\\
24	1.27358169941648e-09\\
25	1.23185534410129e-09\\
26	1.20340274613538e-09\\
27	1.18400193707681e-09\\
28	1.17077402718736e-09\\
30	1.15560717637918e-09\\
32	1.14856190981162e-09\\
36	1.14377546926759e-09\\
46	1.14249329841477e-09\\
100	1.14246525608524e-09\\
};
\addlegendentry{Objective Function (13)}
\end{axis}


\begin{axis}[%
width=5.833in,
height=4.375in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left
]
\end{axis}
\end{tikzpicture}%
